Variability in data streams

We consider the problem of tracking with small relative error an integer function $f(n)$ defined by a distributed update stream $f'(n)$. Existing streaming algorithms with worst-case guarantees for this problem assume $f(n)$ to be monotone; there are very large lower bounds on the space requirements for summarizing a distributed non-monotonic stream, often linear in the size $n$ of the stream. Input streams that give rise to large space requirements are highly variable, making relatively large jumps from one timestep to the next. However, streams often vary slowly in practice. What has heretofore been lacking is a framework for non-monotonic streams that admits algorithms whose worst-case performance is as good as existing algorithms for monotone streams and degrades gracefully for non-monotonic streams as those streams vary more quickly. In this paper we propose such a framework. We introduce a new stream parameter, the "variability" $v$, deriving its definition in a way that shows it to be a natural parameter to consider for non-monotonic streams. It is also a useful parameter. From a theoretical perspective, we can adapt existing algorithms for monotone streams to work for non-monotonic streams, with only minor modifications, in such a way that they reduce to the monotone case when the stream happens to be monotone, and in such a way that we can refine the worst-case communication bounds from $\Theta(n)$ to $\tilde{O}(v)$. From a practical perspective, we demonstrate that $v$ can be small in practice by proving that $v$ is $O(\log f(n))$ for monotone streams and $o(n)$ for streams that are "nearly" monotone or that are generated by random walks. We expect $v$ to be $o(n)$ for many other interesting input classes as well.

==> results/lowerbounds-det.tex <==
\begin{theorem}
  \label{thm:lowerbounds-det}
  Let $\ep = 1 / m$ for some integer $m \ge 2$, let $n \ge 2 m$, let $c < 1$
  constant, and let $r \le n^c$ and even. If a deterministic summary $S(f)$
  guarantees, even only for sequences for which $v(n) = \frac{6 m + 9}{2 m + 6}
  \ep r$, that $|f(t) - \fhat(t)| \le \ep f(t)$ for all $t \le n$, then that
  summary must use $\Omega(\frac{\log n}{\ep} v(n))$ bits of space.
\end{theorem}
\begin{proof}
  We construct a family of input sequences of length $n$ and variability
  $\frac{6 m + 9}{2 m + 6} \ep r$. Choose sets of $r$ different indices $1
  \ldots n$ so that there are $\text{choose}(n,r)$ such sets.

  For each set $S$ we define an input sequence $f_S$. We define $f_S(0) = m$ and
  the rest of $f_S$ recursively: $f_S(t) = f_S(t \m 1)$ if $t$ is not in $S$,
  and $f_S(t) = (2 m + 3) - f_S(t \m 1)$ if $t$ is in $S$. (That is, switch
  between $m$ and $m+3$.)

  If $A$ and $B$ are two different sets, then $f_A \ne f_B$: let $i$ be the
  smallest index that is in one and not the other; say $i$ is in $A$. Then
  $f_A(1 \ldots (i \m 1)) = f_B(1 \ldots (i \m 1))$, but $f_A(i) \ne f_A(i \m 1)
  = f_B(i \m 1) = f_B(i)$.

  The variability of any $f_S$ is $\frac{6 m + 9}{2 m + 6} \ep r$: There are
  $r/2$ changes from $m$ to $m+3$ and another $r/2$ from $m+3$ to $m$. When we
  switch from $m$ to $m+3$, we get $|f'(t)/f(t)| = 3/(m+3)$, and when we switch
  from $m+3$ to $m$, we get $|f'(t)/f(t)| = 3/m$. Thus $\sum_t
  |\frac{f'(t)}{f(t)}| = \frac{r}{2} \frac{6 m + 9}{m (m+3)} = \frac{6 m + 9}{2
    m + 6} \ep r$.

  There are $\text{choose}(n,r) \ge (n/r)^r$ input sequences in our family, so
  to distinguish between any two input sequences we need at least $r \log(n/r) =
  \Omega(r \log n)$ bits. Any summary that can determine for each $t$ the value
  $f(t)$ to within $\pm \ep f(t)$, must also distinguish between $f(t) = m$ and
  $f(t) = m+3$, since there is no value within $\ep m$ of $m$ and also within
  $\ep (m+3)$ of $m+3$. Since this summary must distinguish between $f(t) = m$
  and $f(t) = m+3$ for all $t$, it must distinguish between any two input
  sequences in the family, and therefore needs $\Omega(r \log n)$ bits.
\end{proof}


==> results/lowerbounds-lem0-thm2.tex <==
\begin{lemma}
  Fix some $\ep$. Suppose that the tracing problem has an
  $\Omega(L_{\ep}(n))$-bit space deterministic lower bound. Also suppose that
  there is a deterministic algorithm $A$ for the distributed tracking problem
  that uses $\Omega(C_{\ep}(n))$ bits of communication and $\Omega(S_{\ep}(n))$
  bits of space at the site and coordinator combined. Then we must have $C + S =
  \Omega(L)$.

  Further, if we replace ``deterministic'' with ``randomized'' in the preceding
  paragraph, the claim still holds.
\end{lemma}


==> results/lowerbounds-lem0.tex <==
\begin{lemma}
  \label{lem:lowerbounds-lem0}
  Fix some $\ep$. Suppose that the tracing problem has an
  $\Omega(L_{\ep}(n))$-bit space deterministic lower bound. Also suppose that
  there is a deterministic algorithm $A$ for the distributed tracking problem
  that uses $\Omega(C_{\ep}(n))$ bits of communication and $\Omega(S_{\ep}(n))$
  bits of space at the site and coordinator combined. Then we must have $C + S =
  \Omega(L)$.

  Further, if we replace ``deterministic'' with ``randomized'' in the preceding
  paragraph, the claim still holds.
\end{lemma}
\begin{proof}
  Suppose instead that for all constants $c < 1$ and all $n_0$ there is an $n >
  n_0$ such that $C(n) + S(n) < c L(n)$. Then we can write an algorithm $B$ for
  the tracing problem that uses $L'(n) < c L(n)$ bits of space: simulate $A$,
  recording all communication, and on a query $t$, play back the communication
  that occurred through time $t$.

  At no point did we use the fact that $A$ guarantees $P(|f(t) \m \fhat(t)| \le
  \ep f(t)) = 1$, so the claim still holds if we change the correctness
  requirement to $P \ge 2/3$.
\end{proof}


==> results/lowerbounds-rand-lem1.tex <==
\begin{lemma}
  \label{lem:lowerbounds-rand-lem1}
  Let $\FF$ be a family of sequences of length $n$ and variabilities $\le v$
  such that no two sequences in $\FF$ match. If a summary $S(f)$ guarantees for
  all $f$ in $\FF$ that $P(|f(t) - \fhat(t)| \le \ep f(t)) \;\ge\; 99/100$ for
  all $t \le n$, then that summary must use $\Omega(\log |\FF|)$ bits of space.
\end{lemma}
\begin{proof}
  Let $S(f)$ be the summary for a sequence $f$, and sample $\fhat(1) \ldots
  \fhat(n)$ once each using $S(f)$ to get $\fhat$. Let $A$ be the event that
  $|\{t \::\: |f(t) \m \fhat(t)| \le \ep f(t)\}| \;\ge\; \frac{90}{100} n$. By
  Markov's inequality and the guarantee in the premise, we must have $P(A) \ge
  9/10$.

  Let $\omega$ define the random bits used in constructing $S(f)$ and in
  sampling $\fhat$. For any choice $\omega$ in $A$ we have that $\fhat$ overlaps
  with $f$ in at least $\frac{9}{10} n$ positions, which means that $\fhat$
  overlaps with any other $g \in \FF$ in at most $\frac{7}{10} n$ positions: at
  most the $\frac{6}{10} n$ in which $f$ and $g$ could overlap, plus the
  $\frac{1}{10} n$ in which $\fhat$ and $f$ might not overlap.

  Define $F \subseteq \FF$ to be the sequences $g$ that overlap with $\fhat$ in
  at least $\frac{9}{10} n$ positions. This means that when $\omega \in A$ we
  have $|F| = 1$, and therefore with probability at least $9/10$ we can identify
  which sequence $f$ had been used to construct $S(f)$.

  We now prove our claim by reducing the $\text{Index}_N$ problem to the problem
  of tracing the history of a sequence $f$. The following statement of
  $\text{Index}_N$ is roughly as in Kushilevitz and Nisan \cite{KN1997}. There
  are two parties, Alice and Bob. Alice has an input string $x$ of length $N =
  \log_2 |\FF|$ and Bob has an input string $i$ of length $\log_2 N$ that is
  interpreted as an index into $x$. Alice sends a message to Bob, and then Bob
  must output $x_i$ correctly with probability at least $9/10$.

  Consider the following algorithm for solving $\text{Index}_N$. Alice
  deterministically generates a family $\FF$ of sequences of length $n$ and
  variabilities $\le v$ such that no two match, by iterating over all possible
  sequences and choosing each next one that doesn't match any already chosen.
  Her $\log_2 |\FF|$ bits of input $x$ index a sequence $f$ in $\FF$. Alice
  computes a summary $S(f)$ and sends it to Bob. After receiving $S(f)$, Bob
  computes $\fhat(t)$ for every $t = 1 \ldots n$, to get a sequence $\fhat$. He
  then generates $\FF$ himself and creates a set $F$ of all sequences in $\FF$
  that overlap with $\fhat$ in at least $\frac{9}{10} n$ positions. If $F =
  \{f\}$, which it is with probability at least $9/10$, then Bob can infer every
  bit of $x$.

  Since the $\text{Index}_N$ problem is known to have a one-way communication
  complexity of $\Omega(N)$, it must be that $|S(f)| = \Omega(\log |\FF|)$.
\end{proof}


==> results/lowerbounds-rand-lem2.tex <==
\begin{lemma}
  \label{lem:lowerbounds-rand-lem2}
  For all $\ep \le 1/2$, $v \ge 32400 \ep \ln C$, and $n > 3 v / \ep$, there is
  a family $\FF$ of size $e^{\Omega(v/\ep)}$ of sequences of size $n$ such that:
  \begin{enumerate*}
  \item no two sequences match, and
  \item every sequence has variability at most $v$.
  \end{enumerate*}
\end{lemma}
\begin{proof}
  We construct $\FF$ so that each of the two items holds (separately) with
  probability at least $4/5$. Let $m = 1/\ep$. To construct one sequence in
  $\FF$, first define $f(0) = m$ with probability $1/2$, else $f(0) = m \!+\!
  3$. Then, for $t = 1 \ldots n$: define $f(t) = (2m \!+\! 3) - f(t \m 1)$ with
  probability $p = v/6 \ep n$, else $f(t) = f(t \m 1)$. That is, switch from $m$
  to $m \!+\! 3$ (or vice-versa) with probability $p = v/6 \ep n$.

  We first prove that the probability is at most $1/5$ that any two sequences
  $f$ and $g$ match. We have that $P(f(0) \eq g(0)) = 1/2$. If at any point in
  time we have $f(t) = g(t)$, then $P(f(t \!+\! 1) \eq g(t \!+\! 1)) = \alpha =
  1 - 2 p (1 \m p)$ and $P(f(t \!+\! 1) \!\ne\! g(t \!+\! 1)) = 1 - \alpha = 2 p
  (1 \m p)$. Similarly, if $f(t) \ne g(t)$, then $P(f(t \!+\! 1) \eq g(t \!+\!
  1)) = 1 - \alpha$ and $P(f(t \!+\! 1) \!\ne\! g(t \!+\! 1)) = \alpha$.

  The overlap between $f$ and $g$ is the number of times $t$ that $f(t) = g(t)$.
  We model this situation with a Markov chain $M$ with two states, $c$ for
  ``same'' (that is, $f = g$) and $d$ for ``different'' ($f \ne g$). Let $s_t$
  be the state after $t$ steps, and let $p_t = (p_t(c), p_t(d))$ be the
  probabilities that $M$ is in state $c$ and $d$ after step $t$. The stationary
  distribution $\pi = (1/2, 1/2)$, which also happens to be our initial
  distribution. We can model the overlap between $f$ and $g$ by defining a
  function $y(s_t) = 1$ if $s_t = c$ and $y(s_t) = 0$ otherwise; then $Y =
  \sum_{t = 1}^n y(s_t)$ is the overlap between $f$ and $g$. The expected value
  $E(y(\pi))$ of $y$ evaluated on $\pi$ is $1/2$.

  The $(1/8)$-mixing time $T$ is defined as the smallest time $T$ such that
  $\frac{1}{2}||M^t r_0 - \pi||_1 \le 1/8$ over all initial distributions $r_0$.
  Let $r_0$ be any initial distribution and $r_t = M^t r_0$. If we define
  $\Delta_t = r_t(c) - \pi(c)$, then $\Delta_t = (2 \alpha \m 1)^t \Delta_0$. We
  can similarly bound $|r_t(d) - \pi(d)|$, so we can bound
  \begin{align*}
    T
    \;&\le\; \frac{\ln(8)}{\ln(1/(2 \alpha \m 1))}
    \;\le\; \frac{3}{(1 - (2 \alpha \m 1))}
    \;\le\; \frac{3}{2 p (1 \m p)}
    \;\le\; \frac{3}{2 p}
    \;=\; \frac{9 \ep n}{v}
  \end{align*}
  since $1 - p \ge 1/2$ and since $1/\ln(1/x) \le 1/(1 \m x)$ for $x$ in
  $(0,1)$. With this information we can now apply a sledgehammer of a result by
  Chung, Lam, Liu, and Mitzenmacher \cite{CLLM2012}.
  %
  Our fact \ref{fac:lowerbounds-rand-lem-cllm} is their theorem 3.1, specialized
  a bit to our situation:
  \begin{fact}
    \label{fac:lowerbounds-rand-lem-cllm}
    Let $M$ be an ergodic Markov chain with state space $S$. Let $T$ be its
    $(1/8)$-mixing time. Let $(s_1, \ldots, s_n)$ denote an $n$-step random walk
    on $M$ starting from its stationary distribution $\pi$. Let $y$ be a weight
    function such that $E(y(\pi)) = \mu$. Define the total weight of the walk by
    $Y = \sum_{t = 1}^n y(s_t)$. Then there exists some universal constant $C$
    such that $P(Y \ge (1 + \delta) \mu n) \;\le\; C \exp(-\delta^2 \mu n / 72
    T)$ when $0 < \delta < 1$.
  \end{fact}
  Specifically, this means that $P(Y \ge \frac{6}{10} n) \;\le\; C \exp(-v / (25
  \cdot 72 \cdot 9 \cdot \ep))$. Since $v$ is large enough, we can also write $P
  \le \exp(-v / 32400 \ep)$. If $|\FF| = \frac{1}{5} \exp(v / (2 \cdot 32400
  \ep))$, then by the union bound, with probability at least $4/5$, no pair of
  sequences $f, g$ matches.

  We also must prove that there are enough sequences with variability at most
  $v$. The change in variability due to a single switch from $m$ to $m \!+\! 3$
  (or vice-versa) is at most $3/m = 3 \ep$. For any sequence $f$, let $U_t = 1$
  if $f$ switched at time $t$, else $U_t = 0$. The expected number of switches
  is $v / 6 \ep$; using a standard Chernoff bound, $P(\sum_t U_t \ge 2 v / 6
  \ep) \;\le\; \exp(-v / 18 \ep) \;\le\; 1/10$. Suppose we sample $N$ sequences
  and $B$ of them have more than $2 v / 6 \ep$ switches. In expectation there
  are at most $E(B) \le \frac{1}{10} N$ that have too many switches. By Markov's
  inequality, $P(B \ge N/2) \;\le\; 1/5$, so we can toss out the $\le N/2$ bad
  sequences. This gives us a final size of $\FF$ of $\frac{1}{10} \exp(v / (2
  \cdot 32400 \ep))$.
\end{proof}


==> results/smallvar-biased-thm.tex <==
\begin{theorem}
  \label{thm:smallvar-cases-biased}
  If $f'(t)$ is a sequence of i.i.d. $\pm 1$ random variables with $P(f'(t)
  \!=\! 1) = (1+\mu)/2$ then $E(v(n)) = O(\frac{\log n}{\mu})$.
\end{theorem}


==> results/smallvar-biased.tex <==
\begin{theorem}
  \label{thm:smallvar-cases-biased}
  If $f'(t)$ is a sequence of i.i.d. $\pm 1$ random variables with $P(f'(t)
  \!=\! 1) = (1+\mu)/2$ then $E(v(n)) = O(\frac{\log n}{\mu})$.
\end{theorem}
\begin{proof}
  We show that, with high probability, $f(t) \ge \mu t / 2$ for times $t \ge t_0
  = t_0(n)$ when $n$ is large enough with respect to $\mu$.

  We write $f(t) = -t + 2 Y_t$, where $Y_t = \sum_{s = 1}^t y_s$, and $y_s$ is a
  Bernoulli variable with mean $\frac{1 + \mu}{2}$. We have that $P(f(t) \!\le\!
  \mu t / 2) = P(Y_t \!\le\! \frac{2 + \mu}{4} t)$ and that $E(Y_t) = \frac{1 +
    \mu}{2} t$. Using a Chernoff bound, $P(Y_t \!\le\! \frac{2 + \mu}{4} t) \le
  \exp(-\mu t / 16)$. Let $A$ be the event $\exists t \!\ge\! t_0 \, (f(t) \le
  \mu t / 2)$. Then $P(A) \le \sum_{t = t_0}^n e^{-\mu t / 16}$ by the union
  bound. We can upper bound this sum by
  \begin{align*}
    \sum_{t = t_0}^n e^{-\mu t / 16} \;\le\;
    e^{-\mu t_0 / 16} + \int_{t_0}^n e^{-\mu t / 16} \, dt \;\le\;
    17 e^{-\mu t_0 / 16} / \mu
  \end{align*}
  Taking $t_0 = (16 / \mu) \ln(17 n / \mu)$ gives us $P(A) \le 1/n$. Thus
  \begin{align*}
    E\left(\sum_{t=1}^n \min\{1, |\frac{f'(t)}{f(t)}|\}\right) \;\le\;
    t_0 + \left(\frac{1}{n}\right) n + \left(1 - \frac{1}{n}\right) \sum_{t=t_0}^n \frac{2}{\mu t} \;=\;
    O\left(\frac{\log n}{\mu}\right)
  \end{align*}
  yielding the theorem.
\end{proof}


==> results/smallvar-nearlymonotone-thm.tex <==
\begin{theorem}
  \label{thm:smallvar-cases-nearlymonotone}
  Let $f^-(n) = \sum_{t : f'(t) < 0} |f'(t)|$ and $f^+(n) = \sum_{t : f'(t) > 0}
  f'(t)$. If there is a monotone nondecreasing function $\beta(t) \ge 1$ and a
  constant $t_0$ such that for all $n \ge t_0$ we have $f^-(n) \le \beta(n)
  f(n)$, then the variability $\sum_{t=1}^n |f'(t)/f(t)|$ is $O(\beta(n)
  \log(\beta(n) f(n)))$.
%%   \begin{align*}
%%     \sum_{t=1}^n \frac{|f'(t)|}{f(t)}
%% %
%%     c + 4 (1 + \beta(n)) (1 + \log((1 + \beta(n)) f(n)))
%%   \end{align*}
\end{theorem}


==> results/smallvar-nearlymonotone.tex <==
\input{results/smallvar-nearlymonotone-thm.tex}
\input{results/smallvar-nearlymonotone-proof.tex}

